Finite Element Approximation of Invariant Manifolds by the Parameterization Method

We combine the parameterization method for invariant manifolds with the finite element method for elliptic PDEs,to obtain a new computational framework for high order approximation of invariant manifolds attached to unstable equilibrium solutions of nonlinear parabolic PDEs. The parameterization method provides an infinitesimal invariance equation for the invariant manifold, which we solve via a power series ansatz. A power matching argument leads to a recursive system of linear elliptic PDEs -- the so-called homological equations -- whose solutions are the power series coefficients of the parameterization. The homological equations are solved recursively to any desired order using finite element approximation. The end result is a polynomial expansion for a chart map of the manifold, with coefficients in an appropriate finite element space. We implement the method for a variety of example problems having both polynomial and non-polynomial nonlinearities, on non-convex two-dimensional polygonal domains (not necessary simply connected), for equilibrium solutions with Morse indices one and two. We implement a-posteriori error indicators which provide numerical evidence in support of the claim that the manifolds are computed accurately.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\usepackage{lipsum}
%\usepackage{amsfonts}
%\usepackage{graphicx}
%\usepackage{epstopdf}
%\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{url}

\usepackage{authblk}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{verbatim}
%\usepackage{mathrsfs}
\usepackage{subfigure}
%\usepackage{fancyhdr}
\usepackage{latexsym}
%\usepackage{dsfont}
\usepackage{color}
\usepackage{fancybox}
%\usepackage{framed, color}
%\usepackage[numbers,sort&compress]{natbib}
%
%
%\definecolor{shadecolor}{rgb}{1, 0.8, 0.3}
%
%
%
%\usepackage {blindtext}
\usepackage{geometry}
%\usepackage{fancyhdr}
%\usepackage{amsmath , amsthm , amssymb}
%
%\usepackage{amsfonts}
%\usepackage{graphicx}
\usepackage{hyperref}

\usepackage{mathtools}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\usepackage{mathrsfs}

\usepackage{dsfont}




\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}


\usepackage{dsfont}

\newcommand{\R}{\mathbb R}


% Sets running headers as well as PDF title and authors
\headers{Finite Element Approximation of Invariant Manifolds \\
%by the Parameterization Method
}{
Jorge Gonzalez, J.D. Mireles James, and Necibe Tuncer 
}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Finite Element Approximation of Invariant Manifolds \\
by the Parameterization Method
\thanks{Submitted to the editors DATE.
\funding{J.G. and J.D.M.J. were partially supported by 
the Sloan Foundation Grant FIDDS-17.  J.D.M.J. was partially 
supported by the National Science Foundation grant  DMS - 1813501.}}}
% Authors: full names plus addresses.
\author{Jorge Gonzalez \thanks{School of Mathematics, 
Georgia Institute of Technology, Atlanta, GA
  (\email{jgonzalez35@gatech.edu}, \url{https://people.math.gatech.edu/~jgonzalez35/index.html})}
\and J.D. Mireles James \thanks{Department of Mathematical Sciences, 
Florida Atlantic University, Boca Raton, FL  
   (\email{jmirelesjames@fau.edu}, \url{http://www.math.fau.edu/people/faculty/mirelesjames.php})}
\and Necibe Tuncer  \thanks{Department of Mathematical Sciences, 
Florida Atlantic University, Boca Raton, FL 
  (\email{ntuncer@fau.edu}, \url{http://www.math.fau.edu/people/faculty/tuncer.php})}
}



\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

